Testing Noninterference, Quickly

Information-flow control mechanisms are difficult both to design and to prove correct. To reduce the time wasted on doomed proof attempts due to broken definitions, we advocate modern random testing techniques for finding counterexamples during the design process. We show how to use QuickCheck, a property-based random-testing tool, to guide the design of increasingly complex information-flow abstract machines, leading up to a sophisticated register machine with a novel and highly permissive flow-sensitive dynamic enforcement mechanism that is sound in the presence of first-class public labels. We find that both sophisticated strategies for generating well-distributed random programs and readily falsifiable formulations of noninterference properties are critically important for efficient testing. We propose several approaches and evaluate their effectiveness on a collection of injected bugs of varying subtlety. We also present an effective technique for shrinking large counterexamples to minimal, easily comprehensible ones. Taken together, our best methods enable us to quickly and automatically generate simple counterexamples for more than 45 bugs. Moreover, we show how testing guides the discovery of the sophisticated invariants needed for the noninterference proof of our most complex machine.

==> Makefile <==
PDFLATEX = pdflatex -halt-on-error -synctex=1

NAME = main

all: 
	$(MAKE) once
	$(PDFLATEX) $(NAME)
	$(PDFLATEX) $(NAME)

once: 
	$(PDFLATEX) $(NAME)
	-bibtex $(NAME)
	cp $(NAME).pdf temp.pdf

# You can get pulp here: https://github.com/dmwit/pulp
PULP = "$(shell which pulp || echo \"$(HOME)\"~/.cabal/bin/pulp)"

pulp: $(NAME).tex
	rm -f $(NAME).log
	-$(PDFLATEX) -interaction nonstopmode $< &> /dev/null
	-bibtex $(NAME) | sed -r -e "/Repeated entry---line .* of file safe.bib/,/I'm skipping/ d"
	-$(PDFLATEX) -interaction nonstopmode $< &> /dev/null
	-$(PDFLATEX) -interaction nonstopmode $< &> /dev/null
	-$(PDFLATEX) -interaction nonstopmode $< &> /dev/null
	-$(PULP) $(NAME).log

regenerate:
	$(MAKE) -C ../tmu picotables-fast
	$(MAKE) once

regenerate-sanity-checks:
	$(MAKE) -C ../tmu picotables-fast-sanity-checks
	$(MAKE) once

bcp:
	cp ~/c/safe.bib readonly
	$(MAKE) once

refresh-exp:
	rm exp-*
	$(MAKE) -C ../tmu picotables-fast
	-svn add    `svn status | grep exp- | grep ^?   | cut -c9-`
	-svn rm     `svn status | grep exp- | grep '^!' | cut -c9-`
	-svn revert `svn status | grep exp- | grep ^M   | cut -c9-`

clean:
	@ rm -rf temp* *.aux *.log $(NAME).pdf *.out *.bbl *.blg *.toc *.synctex*

.PHONY : all clean check pulp bib-files

SAFEGIT = /home/hritcu/Penn/safe/git
QCPRIVGIT = /home/hritcu/Inria/quick-chick/priv/latex

# do not try this at home
bib-files:
	cp $(SAFEGIT)/safe.bib readonly
	cp $(QCPRIVGIT)/quick-chick.bib readonly
	svn ci -m "[minor] refreshed bibs" readonly

# normally, there should be no need to do this again
# http://nxg.me.uk/dist/urlbst/
# http://www.tex.ac.uk/tex-archive/biblio/bibtex/contrib/urlbst/urlbst.pdf
regenerate-bib-style: abbrvnatnourl.bst
	urlbst --inlinelinks --hyperref abbrvnatnourl.bst abbrvnaturl.bst

DATE = $(shell date --i)

release-techreport:
	rm -dfr techrep techrep-$(DATE).zip
	mkdir techrep
	cp Makefile techrep
	cp main.tex counter-*.tex exp-*.tex prof*.tex techrep
	cp expsettings.tex genbasic.tex giant-table.tex pico*-names.tex techrep
	cp *.bst *.sty *.bib report.cls techrep
	cp main.log.pulp techrep
	echo "\draftfalse\fulltrue\techreptrue" > techrep/texdirectives.tex
	cp ../../quick-chick.bib techrep
	sed -i 's/\.\.\/\.\.\/quick-chick/quick-chick/g' techrep/main.tex
	cp readonly/safe.bib techrep
	sed -i 's/readonly\///g' techrep/main.tex
	sed -i 's/readonly\\\/safe.bib/safe.bib/g' techrep/Makefile
	make -C techrep pulp
	rm techrep/main.synctex.gz
	rm techrep/*.bib # they explicitly ask for it
	mv techrep/main.pdf techrep-$(DATE).pdf
	cd techrep; zip ../techrep-$(DATE).zip *


==> counter-Basic-EENI-Mem-PushNoTaint.tex <==
% Generator: 1947046545 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{0}{1} \labelsym \high, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{0}{1} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\variation{0}{1} \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[\variation{0}{1} \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 6609, numShrinks = 53


==> counter-basic1.tex <==
% Flags: TMUDriver {gen_instrs = InstrsBasic, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugArithNoTaint,IfcBugPushNoTaint,IfcBugLoadNoTaint,IfcBugStoreNoPointerTaint,IfcBugStoreNoValueTaint,IfcBugAllowWriteDownThroughHighPtr]", ifc_semantics_singleton = [IfcBugArithNoTaint,IfcBugPushNoTaint,IfcBugLoadNoTaint,IfcBugStoreNoPointerTaint,IfcBugStoreNoValueTaint,IfcBugAllowWriteDownThroughHighPtr], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 2004782434 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{0}{1} \labelsym \high, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{0}{1} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\variation{0}{1} \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[\variation{0}{1} \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 1, numShrinks = 116


==> counter-basic2.tex <==
% Flags: TMUDriver {gen_instrs = InstrsBasic, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugArithNoTaint,IfcBugLoadNoTaint,IfcBugStoreNoPointerTaint,IfcBugAllowWriteDownThroughHighPtr]", ifc_semantics_singleton = [IfcBugArithNoTaint,IfcBugLoadNoTaint,IfcBugStoreNoPointerTaint,IfcBugAllowWriteDownThroughHighPtr], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 966669208 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;\variation{0}{1} \labelsym \high, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;\variation{0}{1} \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \high,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[\variation{1}{0} \labelsym \low,\variation{0}{1} \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 1, numShrinks = 123


==> counter-basic3.tex <==
% Flags: TMUDriver {gen_instrs = InstrsBasic, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugArithNoTaint,IfcBugLoadNoTaint,IfcBugAllowWriteDownThroughHighPtr]", ifc_semantics_singleton = [IfcBugArithNoTaint,IfcBugLoadNoTaint,IfcBugAllowWriteDownThroughHighPtr], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 2006423151 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;0 \labelsym \low, \ii{Push}\;\variation{0}{1} \labelsym \high, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;\variation{0}{1} \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \high,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \variation{\high}{\low},0 \labelsym \variation{\low}{\high}\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 1, numShrinks = 118


==> counter-basic4.tex <==
% Flags: TMUDriver {gen_instrs = InstrsBasic, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugArithNoTaint,IfcBugLoadNoTaint]", ifc_semantics_singleton = [IfcBugArithNoTaint,IfcBugLoadNoTaint], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 448074510 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{0}{1} \labelsym \high, \ii{Push}\;0 \labelsym \low, \ii{Add}, \ii{Push}\;0 \labelsym \low, \ii{Store}, \\ \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{0}{1} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \high\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\variation{0}{1} \labelsym \high\right] & \ii{Add} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\variation{0}{1} \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[\variation{0}{1} \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 13, numShrinks = 43


==> counter-basic5.tex <==
% Flags: TMUDriver {gen_instrs = InstrsBasic, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugLoadNoTaint]", ifc_semantics_singleton = [IfcBugLoadNoTaint], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 221979803 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;0 \labelsym \low, \ii{Push}\;1 \labelsym \low, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Push}\;\variation{0}{1} \labelsym \high, \\ \ii{Load}, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[1 \labelsym \low,0 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;\variation{0}{1} \labelsym \high \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \high,0 \labelsym \low\right] & \ii{Load} \\
  \counterexampleline \CEPC{6 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[\variation{1}{0} \labelsym \low,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{7 \labelsym \low} & \left[\variation{1}{0} \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 32, numShrinks = 108


==> counter-basic6.tex <==
% Flags: TMUDriver {gen_instrs = InstrsBasic, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugLoadNoTaint]", ifc_semantics_singleton = [IfcBugLoadNoTaint], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1314609945 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Push}\;0 \labelsym \low, \ii{Push}\;\variation{1}{0} \labelsym \high, \\ \ii{Load}, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;\variation{1}{0} \labelsym \high \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[\variation{1}{0} \labelsym \high,0 \labelsym \low\right] & \ii{Load} \\
  \counterexampleline \CEPC{6 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \low,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{7 \labelsym \low} & \left[\variation{0}{1} \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 70, numShrinks = 157


==> counter-bug1.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugArithNoTaint]", ifc_semantics_singleton = [IfcBugArithNoTaint], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1071801446 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;\variation{0}{1} \labelsym \high, \ii{Push}\;0 \labelsym \low, \ii{Add}, \ii{Store}, \\ \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;\variation{0}{1} \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \high,1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low,\variation{0}{1} \labelsym \high,1 \labelsym \low\right] & \ii{Add} \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[\variation{1}{0} \labelsym \low,\variation{0}{1} \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 23, numShrinks = 95


==> counter-bug10.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugAllowWriteDownWithHighPc]", ifc_semantics_singleton = [IfcBugAllowWriteDownWithHighPc], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1750601535 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;5 \labelsym \low, \ii{Jump}, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Return}\ReturnRet{\False}, \\ \ii{Push}\;0 \labelsym \low, \ii{Push}\;\variation{2}{4} \labelsym \high, \ii{Call}\CallArgs{1}\CallRet{\False}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;5 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[5 \labelsym \low\right] & \ii{Jump} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{6 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;\variation{2}{4} \labelsym \high \\
  \counterexampleline \CEPC{7 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{2}{4} \labelsym \high,0 \labelsym \low\right] & \ii{Call}\CallArgs{1}\CallRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{2 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{8}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{3 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low,\HSret{8}{\False}{\low}\right] & \ii{Store} \\
  \counterexampleline \CEPC{4 \labelsym \high} & \left[0 \labelsym \high\right] & \left[\HSret{8}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{8 \labelsym \low} & \left[0 \labelsym \high\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{4 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{8}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{8 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 468, numShrinks = 167


==> counter-bug11.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugCallNoRaisePc]", ifc_semantics_singleton = [IfcBugCallNoRaisePc], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 772178583 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Push}\;\variation{8}{6} \labelsym \high, \ii{Jump}, \\ \ii{Halt}, \ii{Push}\;10 \labelsym \low, \ii{Call}\CallArgs{0}\CallRet{\False}, \ii{Push}\;5 \labelsym \low, \ii{Call}\CallArgs{0}\CallRet{\False}, \\ \ii{Push}\;0 \labelsym \low, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Return}\ReturnRet{\True}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{8}{6} \labelsym \high \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\variation{8}{6} \labelsym \high\right] & \ii{Jump} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{8 \labelsym \high} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;5 \labelsym \low \\
  \counterexampleline \CEPC{9 \labelsym \high} & \left[1 \labelsym \low\right] & \left[5 \labelsym \low\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\HSret{10}{\False}{\high}\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;10 \labelsym \low \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[1 \labelsym \low\right] & \left[10 \labelsym \low\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \counterexampleline \CEPC{10 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\HSret{8}{\False}{\high}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{11 \labelsym \low} & \left[1 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{8}{\False}{\high}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{12 \labelsym \low} & \left[1 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low,\HSret{8}{\False}{\high}\right] & \ii{Store} \\
  \counterexampleline \CEPC{13 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\HSret{8}{\False}{\high}\right] & \ii{Return}\ReturnRet{\True} \\
  \counterexampleline \CEPC{8 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;5 \labelsym \low \\
  \counterexampleline \CEPC{9 \labelsym \high} & \left[0 \labelsym \low\right] & \left[5 \labelsym \low\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\HSret{10}{\False}{\high}\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 869, numShrinks = 229


==> counter-bug12.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugReturnNoTaint]", ifc_semantics_singleton = [IfcBugReturnNoTaint], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1557352888 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;\variation{6}{7} \labelsym \high, \ii{Call}\CallArgs{1}\CallRet{\True}, \ii{Push}\;0 \labelsym \low, \ii{Store}, \\ \ii{Halt}, \ii{Push}\;0 \labelsym \low, \ii{Return}\ReturnRet{\False}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;\variation{6}{7} \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{6}{7} \labelsym \high,1 \labelsym \low\right] & \ii{Call}\CallArgs{1}\CallRet{\True} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low,\HSret{3}{\True}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low,\HSret{3}{\True}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low,\HSret{3}{\True}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 7537, numShrinks = 905


==> counter-bug13.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugValueOrVoidOnReturn]", ifc_semantics_singleton = [IfcBugValueOrVoidOnReturn], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 128100109 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;0 \labelsym \low, \ii{Push}\;\variation{6}{10} \labelsym \high, \ii{Call}\CallArgs{0}\CallRet{\False}, \ii{Push}\;8 \labelsym \low, \ii{Call}\CallArgs{1}\CallRet{\False}, \\ \ii{Halt}, \ii{Push}\;0 \labelsym \low, \ii{Return}\ReturnRet{\True}, \ii{Push}\;0 \labelsym \low, \ii{Store}, \\ \ii{Return}\ReturnRet{\False}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;\variation{6}{10} \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{6}{10} \labelsym \high,0 \labelsym \low\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{3}{\False}{\low},0 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{3}{\False}{\low},0 \labelsym \low\right] & \ii{Return}\ReturnRet{\True} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \high,0 \labelsym \low\right] & \ii{Push}\;8 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[8 \labelsym \low,0 \labelsym \high,0 \labelsym \low\right] & \ii{Call}\CallArgs{1}\CallRet{\False} \\
  \counterexampleline \CEPC{8 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \high,\HSret{5}{\False}{\low},0 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{9 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \high,\HSret{5}{\False}{\low},0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{10 \labelsym \low} & \left[0 \labelsym \high\right] & \left[\HSret{5}{\False}{\low},0 \labelsym \low\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \high\right] & \left[0 \labelsym \low\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{10 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{3}{\False}{\low},0 \labelsym \low\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;8 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[8 \labelsym \low,0 \labelsym \low\right] & \ii{Call}\CallArgs{1}\CallRet{\False} \\
  \counterexampleline \CEPC{8 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{5}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{9 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low,\HSret{5}{\False}{\low}\right] & \ii{Store} \\
  \counterexampleline \CEPC{10 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\HSret{5}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 35613, numShrinks = 5112


==> counter-bug14.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugPopPopsReturns]", ifc_semantics_singleton = [IfcBugPopPopsReturns], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 10000000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1289838204 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{5}{13} \labelsym \high, \ii{Push}\;1 \labelsym \low, \ii{Store}, \ii{Push}\;15 \labelsym \low, \ii{Jump}, \\ \ii{Push}\;0 \labelsym \low, \ii{Return}\ReturnRet{\False}, \ii{Push}\;0 \labelsym \low, \ii{Push}\;1 \labelsym \low, \ii{Load}, \\ \ii{Call}\CallArgs{0}\CallRet{\True}, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Pop}, \ii{Return}\ReturnRet{\False}, \\ \ii{Push}\;7 \labelsym \low, \ii{Call}\CallArgs{0}\CallRet{\False}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{5}{13} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\variation{5}{13} \labelsym \high\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[1 \labelsym \low,\variation{5}{13} \labelsym \high\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low,\variation{5}{13} \labelsym \high\right] & \left[\,\right] & \ii{Push}\;15 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low,\variation{5}{13} \labelsym \high\right] & \left[15 \labelsym \low\right] & \ii{Jump} \\
  \counterexampleline \CEPC{15 \labelsym \low} & \left[0 \labelsym \low,\variation{5}{13} \labelsym \high\right] & \left[\,\right] & \ii{Push}\;7 \labelsym \low \\
  \counterexampleline \CEPC{16 \labelsym \low} & \left[0 \labelsym \low,\variation{5}{13} \labelsym \high\right] & \left[7 \labelsym \low\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \counterexampleline \CEPC{7 \labelsym \low} & \left[0 \labelsym \low,\variation{5}{13} \labelsym \high\right] & \left[\HSret{17}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{8 \labelsym \low} & \left[0 \labelsym \low,\variation{5}{13} \labelsym \high\right] & \left[0 \labelsym \low,\HSret{17}{\False}{\low}\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{9 \labelsym \low} & \left[0 \labelsym \low,\variation{5}{13} \labelsym \high\right] & \left[1 \labelsym \low,0 \labelsym \low,\HSret{17}{\False}{\low}\right] & \ii{Load} \\
  \counterexampleline \CEPC{10 \labelsym \low} & \left[0 \labelsym \low,\variation{5}{13} \labelsym \high\right] & \left[\variation{5}{13} \labelsym \high,0 \labelsym \low,\HSret{17}{\False}{\low}\right] & \ii{Call}\CallArgs{0}\CallRet{\True} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{5 \labelsym \high} & \left[0 \labelsym \low,5 \labelsym \high\right] & \left[\HSret{11}{\True}{\low},0 \labelsym \low,\HSret{17}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \low,5 \labelsym \high\right] & \left[0 \labelsym \low,\HSret{11}{\True}{\low},0 \labelsym \low,\HSret{17}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{11 \labelsym \low} & \left[0 \labelsym \low,5 \labelsym \high\right] & \left[0 \labelsym \high,0 \labelsym \low,\HSret{17}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{12 \labelsym \low} & \left[0 \labelsym \low,5 \labelsym \high\right] & \left[0 \labelsym \low,0 \labelsym \high,0 \labelsym \low,\HSret{17}{\False}{\low}\right] & \ii{Store} \\
  \counterexampleline \CEPC{13 \labelsym \low} & \left[0 \labelsym \high,5 \labelsym \high\right] & \left[0 \labelsym \low,\HSret{17}{\False}{\low}\right] & \ii{Pop} \\
  \counterexampleline \CEPC{14 \labelsym \low} & \left[0 \labelsym \high,5 \labelsym \high\right] & \left[\HSret{17}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{17 \labelsym \low} & \left[0 \labelsym \high,5 \labelsym \high\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{13 \labelsym \high} & \left[0 \labelsym \low,13 \labelsym \high\right] & \left[\HSret{11}{\True}{\low},0 \labelsym \low,\HSret{17}{\False}{\low}\right] & \ii{Pop} \\
  \counterexampleline \CEPC{14 \labelsym \high} & \left[0 \labelsym \low,13 \labelsym \high\right] & \left[0 \labelsym \low,\HSret{17}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{17 \labelsym \low} & \left[0 \labelsym \low,13 \labelsym \high\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 402009, numShrinks = 40364


==> counter-bug2.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugPushNoTaint]", ifc_semantics_singleton = [IfcBugPushNoTaint], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1778485319 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{0}{1} \labelsym \high, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{0}{1} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\variation{0}{1} \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[\variation{0}{1} \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 4, numShrinks = 63


==> counter-bug3.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugLoadNoTaint]", ifc_semantics_singleton = [IfcBugLoadNoTaint], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 926540483 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Push}\;\variation{0}{1} \labelsym \high, \ii{Load}, \\ \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{0}{1} \labelsym \high \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \high\right] & \ii{Load} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[\variation{1}{0} \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{6 \labelsym \low} & \left[1 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low,\variation{1}{0} \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{7 \labelsym \low} & \left[\variation{1}{0} \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 683, numShrinks = 215


==> counter-bug4.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugStoreNoPointerTaint]", ifc_semantics_singleton = [IfcBugStoreNoPointerTaint], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1965117020 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;0 \labelsym \high, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Push}\;0 \labelsym \low, \ii{Push}\;0 \labelsym \high, \\ \ii{Push}\;1 \labelsym \low, \ii{Store}, \ii{Push}\;\variation{1}{0} \labelsym \high, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;0 \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \high\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \high\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \high,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \high,0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;0 \labelsym \high \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \high,0 \labelsym \low\right] & \left[0 \labelsym \high,0 \labelsym \low\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{6 \labelsym \low} & \left[0 \labelsym \high,0 \labelsym \low\right] & \left[1 \labelsym \low,0 \labelsym \high,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{7 \labelsym \low} & \left[0 \labelsym \high,0 \labelsym \high\right] & \left[0 \labelsym \low\right] & \ii{Push}\;\variation{1}{0} \labelsym \high \\
  \counterexampleline \CEPC{8 \labelsym \low} & \left[0 \labelsym \high,0 \labelsym \high\right] & \left[\variation{1}{0} \labelsym \high,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{9 \labelsym \low} & \left[0 \labelsym \variation{\high}{\low},0 \labelsym \variation{\low}{\high}\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 47297, numShrinks = 238


==> counter-bug5.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugAllowWriteDownThroughHighPtr]", ifc_semantics_singleton = [IfcBugAllowWriteDownThroughHighPtr], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1632210355 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;0 \labelsym \low, \ii{Push}\;\variation{1}{0} \labelsym \high, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;\variation{1}{0} \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\variation{1}{0} \labelsym \high,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \variation{\low}{\high},0 \labelsym \variation{\high}{\low}\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 3, numShrinks = 44


==> counter-bug6.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugStoreNoValueTaint]", ifc_semantics_singleton = [IfcBugStoreNoValueTaint], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 607893934 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{0}{1} \labelsym \high, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{0}{1} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{0}{1} \labelsym \high\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\variation{0}{1} \labelsym \high\right] & \ii{Store} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[\variation{0}{1} \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 14, numShrinks = 53


==> counter-bug7.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugJumpNoRaisePc]", ifc_semantics_singleton = [IfcBugJumpNoRaisePc], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 882497153 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;0 \labelsym \low, \ii{Push}\;\variation{4}{5} \labelsym \high, \ii{Jump}, \ii{Store}, \\ \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Push}\;\variation{4}{5} \labelsym \high \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{4}{5} \labelsym \high,0 \labelsym \low,1 \labelsym \low\right] & \ii{Jump} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 62, numShrinks = 109


==> counter-bug8.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugJumpLowerPc]", ifc_semantics_singleton = [IfcBugJumpLowerPc], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 638333793 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;\variation{5}{6} \labelsym \high, \ii{Jump}, \ii{Store}, \ii{Halt}, \\ \ii{Push}\;0 \labelsym \low, \ii{Push}\;0 \labelsym \low, \ii{Push}\;3 \labelsym \low, \ii{Jump}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;\variation{5}{6} \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{5}{6} \labelsym \high,1 \labelsym \low\right] & \ii{Jump} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{5 \labelsym \high} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low,1 \labelsym \low\right] & \ii{Push}\;3 \labelsym \low \\
  \counterexampleline \CEPC{8 \labelsym \high} & \left[0 \labelsym \low\right] & \left[3 \labelsym \low,0 \labelsym \low,0 \labelsym \low,1 \labelsym \low\right] & \ii{Jump} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Push}\;3 \labelsym \low \\
  \counterexampleline \CEPC{8 \labelsym \high} & \left[0 \labelsym \low\right] & \left[3 \labelsym \low,0 \labelsym \low,1 \labelsym \low\right] & \ii{Jump} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 22747, numShrinks = 3320


==> counter-bug9.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugStoreNoPcTaint]", ifc_semantics_singleton = [IfcBugStoreNoPcTaint], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 2096562579 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{6}{9} \labelsym \high, \ii{Push}\;0 \labelsym \high, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Call}\CallArgs{0}\CallRet{\False}, \\ \ii{Halt}, \ii{Push}\;0 \labelsym \low, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Return}\ReturnRet{\True}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{6}{9} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{6}{9} \labelsym \high\right] & \ii{Push}\;0 \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \high,\variation{6}{9} \labelsym \high\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \high,\variation{6}{9} \labelsym \high\right] & \ii{Store} \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \high\right] & \left[\variation{6}{9} \labelsym \high\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \high\right] & \left[\HSret{5}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \high\right] & \left[0 \labelsym \low,\HSret{5}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{8 \labelsym \high} & \left[0 \labelsym \high\right] & \left[0 \labelsym \low,0 \labelsym \low,\HSret{5}{\False}{\low}\right] & \ii{Store} \\
  \counterexampleline \CEPC{9 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{5}{\False}{\low}\right] & \ii{Return}\ReturnRet{\True} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{9 \labelsym \high} & \left[0 \labelsym \high\right] & \left[\HSret{5}{\False}{\low}\right] & \ii{Return}\ReturnRet{\True} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \high\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 4348, numShrinks = 555


==> counter-cally1.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugStoreNoPcTaint,IfcBugAllowWriteDownWithHighPc,IfcBugReturnNoTaint,IfcBugValueOrVoidOnReturn,IfcBugPopPopsReturns]", ifc_semantics_singleton = [IfcBugStoreNoPcTaint,IfcBugAllowWriteDownWithHighPc,IfcBugReturnNoTaint,IfcBugValueOrVoidOnReturn,IfcBugPopPopsReturns], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 892892905 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{3}{6} \labelsym \high, \ii{Call}\CallArgs{0}\CallRet{\False}, \ii{Halt}, \ii{Push}\;1 \labelsym \low, \ii{Push}\;0 \labelsym \low, \\ \ii{Store}, \ii{Return}\ReturnRet{\False}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{3}{6} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{3}{6} \labelsym \high\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{3 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{2}{\False}{\low}\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \high} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low,\HSret{2}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{5 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low,\HSret{2}{\False}{\low}\right] & \ii{Store} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[1 \labelsym \low\right] & \left[\HSret{2}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{2}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 1098, numShrinks = 774


==> counter-cally2.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugAllowWriteDownWithHighPc,IfcBugReturnNoTaint,IfcBugValueOrVoidOnReturn,IfcBugPopPopsReturns]", ifc_semantics_singleton = [IfcBugAllowWriteDownWithHighPc,IfcBugReturnNoTaint,IfcBugValueOrVoidOnReturn,IfcBugPopPopsReturns], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1106868607 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{3}{6} \labelsym \high, \ii{Call}\CallArgs{0}\CallRet{\False}, \ii{Halt}, \ii{Push}\;0 \labelsym \low, \ii{Push}\;0 \labelsym \low, \\ \ii{Store}, \ii{Return}\ReturnRet{\False}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{3}{6} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{3}{6} \labelsym \high\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{3 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{2}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{2}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{5 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low,\HSret{2}{\False}{\low}\right] & \ii{Store} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \high\right] & \left[\HSret{2}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \high\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{2}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 721, numShrinks = 488


==> counter-cally3.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugReturnNoTaint,IfcBugValueOrVoidOnReturn,IfcBugPopPopsReturns]", ifc_semantics_singleton = [IfcBugReturnNoTaint,IfcBugValueOrVoidOnReturn,IfcBugPopPopsReturns], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1138769688 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;\variation{7}{6} \labelsym \high, \ii{Call}\CallArgs{1}\CallRet{\False}, \ii{Push}\;0 \labelsym \low, \ii{Store}, \\ \ii{Halt}, \ii{Push}\;0 \labelsym \low, \ii{Return}\ReturnRet{\True}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;\variation{7}{6} \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{7}{6} \labelsym \high,1 \labelsym \low\right] & \ii{Call}\CallArgs{1}\CallRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low,\HSret{3}{\False}{\low}\right] & \ii{Return}\ReturnRet{\True} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low,\HSret{3}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low,\HSret{3}{\False}{\low}\right] & \ii{Return}\ReturnRet{\True} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 5088, numShrinks = 10661

==> counter-cally4.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugValueOrVoidOnReturn,IfcBugPopPopsReturns]", ifc_semantics_singleton = [IfcBugValueOrVoidOnReturn,IfcBugPopPopsReturns], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1657060615 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;0 \labelsym \low, \ii{Push}\;\variation{6}{7} \labelsym \high, \ii{Call}\CallArgs{0}\CallRet{\False}, \ii{Push}\;0 \labelsym \low, \ii{Store}, \\ \ii{Halt}, \ii{Return}\ReturnRet{\False}, \ii{Push}\;0 \labelsym \low, \ii{Return}\ReturnRet{\True}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;\variation{6}{7} \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{6}{7} \labelsym \high,0 \labelsym \low\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{3}{\False}{\low},0 \labelsym \low\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{3}{\False}{\low},0 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{8 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{3}{\False}{\low},0 \labelsym \low\right] & \ii{Return}\ReturnRet{\True} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \high,0 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \high,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \high\right] & \left[0 \labelsym \low\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 515, numShrinks = 298


==> counter-cally5.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugPopPopsReturns]", ifc_semantics_singleton = [IfcBugPopPopsReturns], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 66987814 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;5 \labelsym \low, \ii{Call}\CallArgs{0}\CallRet{\True}, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Halt}, \\ \ii{Push}\;0 \labelsym \low, \ii{Push}\;\variation{8}{9} \labelsym \high, \ii{Call}\CallArgs{0}\CallRet{\False}, \ii{Pop}, \ii{Push}\;0 \labelsym \low, \\ \ii{Return}\ReturnRet{\False}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;5 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[5 \labelsym \low\right] & \ii{Call}\CallArgs{0}\CallRet{\True} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\HSret{2}{\True}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{6 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{2}{\True}{\low}\right] & \ii{Push}\;\variation{8}{9} \labelsym \high \\
  \counterexampleline \CEPC{7 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{8}{9} \labelsym \high,0 \labelsym \low,\HSret{2}{\True}{\low}\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{8 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{8}{\False}{\low},0 \labelsym \low,\HSret{2}{\True}{\low}\right] & \ii{Pop} \\
  \counterexampleline \CEPC{9 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{2}{\True}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{10 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low,\HSret{2}{\True}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \high\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \high\right] & \ii{Store} \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \high\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{9 \labelsym \high} & \left[0 \labelsym \low\right] & \left[\HSret{8}{\False}{\low},0 \labelsym \low,\HSret{2}{\True}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{10 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{8}{\False}{\low},0 \labelsym \low,\HSret{2}{\True}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{8 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{2}{\True}{\low}\right] & \ii{Pop} \\
  \counterexampleline \CEPC{9 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\HSret{2}{\True}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{10 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,\HSret{2}{\True}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 45009, numShrinks = 62


==> counter-eeni-no-low.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[]", ifc_semantics_singleton = [], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENInoLow, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1412921613 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{2}{3} \labelsym \high, \ii{Call}\CallArgs{0}\CallRet{\False}, \ii{Halt}, \ii{Return}\ReturnRet{\True}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[\,\right] & \left[\,\right] & \ii{Push}\;\variation{2}{3} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[\,\right] & \left[\variation{2}{3} \labelsym \high\right] & \ii{Call}\CallArgs{0}\CallRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{2 \labelsym \high} & \left[\,\right] & \left[\HSret{2}{\False}{\low}\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{3 \labelsym \high} & \left[\,\right] & \left[\HSret{2}{\False}{\low}\right] & \ii{Return}\ReturnRet{\True} \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[\,\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 185, numShrinks = 100


==> counter-extended-stack-2.tex <==
% Hand-written by Leo, TeXed by Antal
\begin{tabular}{mlmlmlmlml}
  \multicolumn{5}{mc}{i = \left[\OpBRET \right]} \\
  \addlinespace\toprule
  \pc & m & r & s & i(\pc) \\
  \midrule
  \multicolumn{5}{l}{Machine 1's trace\ldots} \\
  \counterexampleline \CEPC{0 \labelsym \low} & \left[\,\right] & \left(\,\right) & \left[\{\retsym\;0 \labelsym \high, \ldots\}, \{\retsym\;0 \labelsym \low, \ldots\}\right] & \OpBRET \\
  \counterexampleline \CEPC{0 \labelsym \high} & \left[\,\right] & \left(\,\right) & \left[\{\retsym\;0 \labelsym \low, \ldots\}\right] & \OpBRET \\
  \midrule
  \multicolumn{5}{l}{Machine 2's trace\ldots} \\
  \counterexampleline \CEPC{0 \labelsym \low} & \left[\,\right] & \left(\,\right) & \left[\{\retsym\;0 \labelsym \low, \ldots\}\right] & \OpBRET \\
  \counterexampleline \CEPC{0 \labelsym \low} & \left[\,\right] & \left(\,\right) & \left[\,\right] & \OpBRET \\
\end{tabular}


==> counter-extended-stack.tex <==
% Hand-written by Leo, TeXed by Antal
\begin{tabular}{mlmlmlmlml}
  \multicolumn{5}{mc}{i = \left[\OpBCALL\;0\;1\;0, \OpBCALL\;0\;2\;0\right]} \\
  \addlinespace\toprule
  \pc & m & r & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \midl_1} & \left[\,\right] & \left(1 \labelsym \low, \variation{\midl_1}{\midl_2} \labelsym \midl_2, \low \labelsym \low\right) & \left[\,\right] & \OpBCALL\;0\;1\;0 \\
  \counterexampleline \CEPC{1 \labelsym \midl_1} & \left[\,\right] & \left(1 \labelsym \low, \variation{\midl_1}{\midl_2} \labelsym \midl_2, \low \labelsym \low\right) & \left[\{\retsym\;1 \labelsym \high, \variation{\midl_1}{\midl_2}, \ldots\}\right] & \OpBCALL\;0\;2\;0 \\
  \counterexampleline \CEPC{1 \labelsym \midl_1} & \left[\,\right] & \left(1 \labelsym \low, \variation{\midl_1}{\midl_2} \labelsym \midl_2, \low \labelsym \low\right) & \left[\{\retsym\;2 \labelsym \midl_1, \low, \ldots\}, \{\retsym\;1 \labelsym \high, \variation{\midl_1}{\midl_2}, \ldots\}\right] & \OpBCALL\;0\;2\;0 \\
\end{tabular}
% Original:
%
% Obs: M1 
%
% PC  : 0 @ M1
% IMem: [BCall 0 1 0, BCall 0 2 0]
% Mem : []
% Regs: 0: VInt 1 @ L
%       1: VLab _ @ M2
%       2: VLab _ @ L
% Stk : []
%
%     
% After one step: 
%
% PC: 1 @ M1
% Stack: [ { RetPC: 1 @ H, ...} ]
%
% After two steps: 
%
% PC: 1 @ M1 
% Stack: [ { RetPC: 2 @ M1, ...} ; { RetPC: 1 @ H, ...} ]


==> counter-high-equiv-everything.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, atom_equiv = HighEquivEverything, ifc_semantics = "[]", ifc_semantics_singleton = [], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1348206757 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;0 \labelsym \high, \ii{Push}\;1 \labelsym \low, \ii{Store}, \ii{Push}\;\variation{1 \labelsym \high}{0 \labelsym \low}, \\ \ii{Store}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[0 \labelsym \high,1 \labelsym \low\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \low\right] & \left[1 \labelsym \low,0 \labelsym \high,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \high\right] & \left[1 \labelsym \low\right] & \ii{Push}\;\variation{1 \labelsym \high}{0 \labelsym \low} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low,0 \labelsym \high\right] & \left[\variation{1 \labelsym \high}{0 \labelsym \low},1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{6 \labelsym \low} & \left[\variation{0}{1} \labelsym \low,\variation{1}{0} \labelsym \high\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 838, numShrinks = 151


==> counter-jumpy1.tex <==
% Flags: TMUDriver {gen_instrs = InstrsJumpy, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugJumpNoRaisePc,IfcBugJumpLowerPc,IfcBugStoreNoPcTaint,IfcBugAllowWriteDownWithHighPc]", ifc_semantics_singleton = [IfcBugJumpNoRaisePc,IfcBugJumpLowerPc,IfcBugStoreNoPcTaint,IfcBugAllowWriteDownWithHighPc], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1099943983 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;\variation{2}{5} \labelsym \high, \ii{Jump}, \ii{Push}\;1 \labelsym \low, \ii{Push}\;0 \labelsym \low, \ii{Store}, \\ \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;\variation{2}{5} \labelsym \high \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{2}{5} \labelsym \high\right] & \ii{Jump} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 4, numShrinks = 51


==> counter-jumpy2.tex <==
% Flags: TMUDriver {gen_instrs = InstrsJumpy, gen_strategy = GenByExec, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, if_labels_observable = True, ifc_semantics = "[IfcBugJumpLowerPc,IfcBugStoreNoPcTaint,IfcBugAllowWriteDownWithHighPc]", ifc_semantics_singleton = [IfcBugJumpLowerPc,IfcBugStoreNoPcTaint,IfcBugAllowWriteDownWithHighPc], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 100, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 1157804124 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;\variation{4}{6} \labelsym \high, \ii{Jump}, \ii{Halt}, \ii{Push}\;0 \labelsym \low, \\ \ii{Store}, \ii{Push}\;3 \labelsym \low, \ii{Jump}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;\variation{4}{6} \labelsym \high \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\variation{4}{6} \labelsym \high,1 \labelsym \low\right] & \ii{Jump} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{4 \labelsym \high} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{5 \labelsym \high} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;3 \labelsym \low \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[1 \labelsym \low\right] & \left[3 \labelsym \low\right] & \ii{Jump} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[1 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{6 \labelsym \high} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;3 \labelsym \low \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \low\right] & \left[3 \labelsym \low,1 \labelsym \low\right] & \ii{Jump} \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 61, numShrinks = 89


==> counter-not-observable.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartInitial, equiv = EquivMem, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, atom_equiv = LabelsNotObservable, ifc_semantics = "[]", ifc_semantics_singleton = [], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 587675921 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Push}\;1 \labelsym \low, \ii{Push}\;0 \labelsym \variation{\high}{\low}, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Push}\;\variation{7}{9} \labelsym \high, \\ \ii{Call}\CallArgs{1}\CallRet{\False}, \ii{Halt}, \ii{Push}\;0 \labelsym \low, \ii{Store}, \ii{Return}\ReturnRet{\False}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Push}\;1 \labelsym \low \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \variation{\high}{\low} \\
  \counterexampleline \CEPC{2 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \variation{\high}{\low},1 \labelsym \low\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{3 \labelsym \low} & \left[0 \labelsym \low\right] & \left[0 \labelsym \low,0 \labelsym \variation{\high}{\low},1 \labelsym \low\right] & \ii{Store} \\
  \counterexampleline \CEPC{4 \labelsym \low} & \left[0 \labelsym \variation{\high}{\low}\right] & \left[1 \labelsym \low\right] & \ii{Push}\;\variation{7}{9} \labelsym \high \\
  \counterexampleline \CEPC{5 \labelsym \low} & \left[0 \labelsym \variation{\high}{\low}\right] & \left[\variation{7}{9} \labelsym \high,1 \labelsym \low\right] & \ii{Call}\CallArgs{1}\CallRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{7 \labelsym \high} & \left[0 \labelsym \high\right] & \left[1 \labelsym \low,\HSret{6}{\False}{\low}\right] & \ii{Push}\;0 \labelsym \low \\
  \counterexampleline \CEPC{8 \labelsym \high} & \left[0 \labelsym \high\right] & \left[0 \labelsym \low,1 \labelsym \low,\HSret{6}{\False}{\low}\right] & \ii{Store} \\
  \counterexampleline \CEPC{9 \labelsym \high} & \left[1 \labelsym \high\right] & \left[\HSret{6}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{6 \labelsym \low} & \left[1 \labelsym \high\right] & \left[\,\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{9 \labelsym \high} & \left[0 \labelsym \low\right] & \left[1 \labelsym \low,\HSret{6}{\False}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{6 \labelsym \low} & \left[0 \labelsym \low\right] & \left[\,\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 20772, numShrinks = 8509


==> counter-ssni-equivlow-too-weak.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenTinySSNI, gen_instrs_range = (20,50), starting_as = StartArbitrary, equiv = EquivLow, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, atom_equiv = LabelsObservable, ifc_semantics = "[]", ifc_semantics_singleton = [], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropSSNI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 10431986 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Return}\ReturnRet{\True}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \high} & \left[\,\right] & \left[\HSret{\variation{0}{1}}{\False}{\low}\right] & \ii{Return}\ReturnRet{\True} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{0 \labelsym \low} & \left[\,\right] & \left[\,\right] & \ii{Return}\ReturnRet{\True} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[\,\right] & \left[\,\right] & \mathord{-} \\
\end{tabular}
% *** Falsifiable, numTests = 497, numShrinks = 45


==> counter-ssni-equivwrongfull.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenTinySSNI, gen_instrs_range = (20,50), starting_as = StartArbitrary, equiv = EquivWrongFull, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, atom_equiv = LabelsObservable, ifc_semantics = "[]", ifc_semantics_singleton = [], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropSSNI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 526966048 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Pop}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \high} & \left[\,\right] & \left[0 \labelsym \low\right] & \ii{Pop} \\
  \counterexampleline \CEPC{1 \labelsym \high} & \left[\,\right] & \left[\,\right] & \mathord{-} \\
\end{tabular}
% *** Falsifiable, numTests = 4, numShrinks = 9


==> counter-stk-elt-equiv-label-on-top.tex <==
% Flags: TMUDriver {gen_instrs = InstrsCally, gen_strategy = GenByExec2, gen_instrs_range = (20,50), starting_as = StartQuasiInitial, equiv = EquivLow, smart_ints = True, shrink_nothing = False, shrink_to_noop = True, shrink_noops = True, atom_equiv = LabelsObservable, stk_elt_equiv = LabelOnTop, ifc_semantics = "[]", ifc_semantics_singleton = [], which_tmm_routine = NoTMMRoutine, tmu_abstract_steps = 50, tmu_concrete_steps = 5000, tmu_timeout = 1, tmu_max_tests = 100000, tmu_max_discard_ratio = 30, tmu_prop_test = PropEENI, tmu_extrapol_mul = 10, tmu_extrapol_add = 1000, show_counterexamples = True, conf_max_call_args = 2, latex_output = True, run_timeout_tests = False}
% Generator: 653803404 2147483398
\begin{tabular}{mlmlmlml}
  \multicolumn{4}{mc}{i = \left[\begin{array}{l}\ii{Return}\ReturnRet{\False}, \ii{Halt}\end{array}\right]} \\
  \addlinespace\toprule
  \pc & m & s & i(\pc) \\
  \midrule
  \counterexampleline \CEPC{0 \labelsym \low} & \left[\,\right] & \left[0 \labelsym \low,\variation{0 \labelsym \high}{\HSret{0}{\False}{\high}},0 \labelsym \low,\HSret{1}{\True}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \midrule
  \multicolumn{4}{l}{Machine 1 continues\ldots} \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[\,\right] & \left[0 \labelsym \low\right] & \ii{Halt} \\
  \midrule
  \multicolumn{4}{l}{Machine 2 continues\ldots} \\
  \counterexampleline \CEPC{0 \labelsym \high} & \left[\,\right] & \left[0 \labelsym \low,\HSret{1}{\True}{\low}\right] & \ii{Return}\ReturnRet{\False} \\
  \counterexampleline \CEPC{1 \labelsym \low} & \left[\,\right] & \left[0 \labelsym \high\right] & \ii{Halt} \\
\end{tabular}
% *** Falsifiable, numTests = 4063, numShrinks = 2098


==> exp-Basic-EENI-Mem-Initial-ByExec-True.tex <==
\gdef\bugtableinfo{../picopaper/exp-Basic-EENI-Mem-Initial-ByExec-True.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{3313}{5\%}{0.87 (E)}{37193}{11.03}{}
\row{\IfcBugPushNoTaint}{3332}{4\%}{0.01 (E)}{307109}{0.02}{}
\row{\IfcBugLoadNoTaint}{3203}{5\%}{4.03 (E)}{17257}{104.89}{}
\row{\IfcBugStoreNoPointerTaint}{3134}{5\%}{1233.51 (A)}{241}{1783964.08}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{3379}{4\%}{0.25 (E)}{69920}{1.46}{}
\row{\IfcBugStoreNoValueTaint}{3345}{3\%}{0.02 (E)}{281139}{0.03}{}
\means{}{206.45}{0.77}{0.04}
\extrabuginfo{InstrsBasic}{\PropEENI}{EquivMem}{StartInitial}{\GenByExec}{True}{300sec}{4000}{Thu Mar 28 18:13:12 EDT 2013}
\averagespeed{3284}
\averagediscrate{4\%}


==> exp-Basic-EENI-Mem-Initial-Naive-False.tex <==
\gdef\bugtableinfo{../picopaper/exp-Basic-EENI-Mem-Initial-Naive-False.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{24245}{79\%}{83247.01 (A)}{3}{1684542577.46}{}
\row{\IfcBugPushNoTaint}{24333}{79\%}{3552.54 (A)}{83}{8898873.25}{}
\row{\IfcBugLoadNoTaint}{23878}{79\%}{---}{0}{---}{}
\row{\IfcBugStoreNoPointerTaint}{23741}{79\%}{---}{0}{---}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{24323}{79\%}{47365.97 (A)}{6}{1869377671.92}{}
\row{\IfcBugStoreNoValueTaint}{24255}{79\%}{7660.07 (A)}{38}{46504022.78}{}
\means{}{---}{---}{8985.53}
\extrabuginfo{InstrsBasic}{\PropEENI}{EquivMem}{StartInitial}{\GenNaive}{False}{300sec}{4000}{Thu Mar 28 18:22:12 EDT 2013}
\averagespeed{24129}
\averagediscrate{79\%}


==> exp-Basic-EENI-Mem-Initial-Sequence-False.tex <==
\gdef\bugtableinfo{../picopaper/exp-Basic-EENI-Mem-Initial-Sequence-False.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{8443}{65\%}{561.58 (A)}{534}{344300.85}{}
\row{\IfcBugPushNoTaint}{8557}{66\%}{0.21 (E)}{75086}{1.18}{}
\row{\IfcBugLoadNoTaint}{8424}{65\%}{73115.63 (A)}{4}{1056385405.49}{}
\row{\IfcBugStoreNoPointerTaint}{8385}{65\%}{38036.22 (A)}{1}{---}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{8520}{64\%}{0.85 (E)}{37576}{8.16}{}
\row{\IfcBugStoreNoValueTaint}{8919}{66\%}{0.41 (E)}{54302}{3.55}{}
\means{}{18619.15}{69.73}{0.72}
\extrabuginfo{InstrsBasic}{\PropEENI}{EquivMem}{StartInitial}{\GenSequence}{False}{300sec}{4000}{Thu Mar 28 18:08:20 EDT 2013}
\averagespeed{8541}
\averagediscrate{65\%}


==> exp-Basic-EENI-Mem-Initial-Sequence-True.tex <==
\gdef\bugtableinfo{../picopaper/exp-Basic-EENI-Mem-Initial-Sequence-True.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{7953}{60\%}{30.05 (E)}{6319}{1480.74}{}
\row{\IfcBugPushNoTaint}{7704}{59\%}{0.07 (E)}{134009}{0.21}{}
\row{\IfcBugLoadNoTaint}{7916}{59\%}{2258.93 (A)}{132}{6629663.72}{}
\row{\IfcBugStoreNoPointerTaint}{7935}{60\%}{32227.10 (A)}{9}{795478324.70}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{7650}{57\%}{0.12 (E)}{98919}{0.51}{}
\row{\IfcBugStoreNoValueTaint}{8330}{62\%}{0.31 (E)}{61871}{2.28}{}
\means{}{5752.76}{13.33}{0.23}
\extrabuginfo{InstrsBasic}{\PropEENI}{EquivMem}{StartInitial}{\GenSequence}{True}{300sec}{4000}{Thu Mar 28 18:06:01 EDT 2013}
\averagespeed{7915}
\averagediscrate{59\%}


==> exp-Basic-EENI-Mem-Initial-Weighted-False.tex <==
\gdef\bugtableinfo{../picopaper/exp-Basic-EENI-Mem-Initial-Weighted-False.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{11549}{62\%}{5344.26 (A)}{56}{43505825.65}{}
\row{\IfcBugPushNoTaint}{11483}{62\%}{309.20 (A)}{969}{90957.16}{}
\row{\IfcBugLoadNoTaint}{11431}{62\%}{---}{0}{---}{}
\row{\IfcBugStoreNoPointerTaint}{11385}{62\%}{---}{0}{---}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{11443}{62\%}{1713.72 (A)}{175}{3718177.41}{}
\row{\IfcBugStoreNoValueTaint}{11503}{62\%}{426.11 (A)}{704}{177746.41}{}
\means{}{---}{---}{629.76}
\extrabuginfo{InstrsBasic}{\PropEENI}{EquivMem}{StartInitial}{\GenWeighted}{False}{300sec}{4000}{Thu Mar 28 18:22:13 EDT 2013}
\averagespeed{11466}
\averagediscrate{62\%}


==> exp-Cally-EENI-Low-Initial-ByExec2-True.tex <==
\gdef\bugtableinfo{../picopaper/exp-Cally-EENI-Low-Initial-ByExec2-True.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{2832}{67\%}{2.38 (E)}{22438}{57.68}{}
\row{\IfcBugPushNoTaint}{2774}{59\%}{0.02 (E)}{244686}{0.05}{}
\row{\IfcBugLoadNoTaint}{2811}{66\%}{37.50 (E)}{5657}{1692.27}{}
\row{\IfcBugStoreNoPointerTaint}{2722}{65\%}{18658.56 (A)}{15}{511296867.51}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{2906}{67\%}{12.87 (E)}{9657}{303.15}{}
\row{\IfcBugStoreNoValueTaint}{3032}{67\%}{0.34 (E)}{59239}{2.59}{}
\row{\IfcBugJumpNoRaisePc}{2860}{62\%}{7.58 (E)}{12586}{269.30}{}
\row{\IfcBugJumpLowerPc}{2794}{65\%}{158.36 (A)}{1894}{27372.02}{}
\row{\IfcBugStoreNoPcTaint}{2762}{65\%}{12295.65 (A)}{23}{89863681.47}{}
\row{\IfcBugAllowWriteDownWithHighPc}{2735}{65\%}{1129.48 (A)}{265}{1129213.01}{}
\row{\IfcBugCallNoRaisePc}{2761}{65\%}{174.66 (A)}{1717}{30037.47}{}
\row{\IfcBugReturnNoTaint}{2748}{65\%}{4698.17 (A)}{63}{21077804.79}{}
\row{\IfcBugValueOrVoidOnReturn}{2744}{65\%}{6940.67 (A)}{43}{62179547.46}{}
\row{\IfcBugPopPopsReturns}{2674}{65\%}{51753.13 (A)}{1}{---}{}
\means{}{6847.81}{135.76}{0.26}
\extrabuginfo{InstrsCally}{\PropEENI}{EquivLow}{StartInitial}{\GenByExec2}{True}{300sec}{4000}{Thu Mar 28 19:01:59 EDT 2013}
\averagespeed{2797}
\averagediscrate{65\%}


==> exp-Cally-EENI-Low-QuasiInitial-ByExec2-True.tex <==
\gdef\bugtableinfo{../picopaper/exp-Cally-EENI-Low-QuasiInitial-ByExec2-True.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{2748}{70\%}{1.38 (E)}{29490}{25.77}{}
\row{\IfcBugPushNoTaint}{2684}{61\%}{0.02 (E)}{221845}{0.06}{}
\row{\IfcBugLoadNoTaint}{2653}{70\%}{5.73 (E)}{14471}{121.31}{}
\row{\IfcBugStoreNoPointerTaint}{2244}{70\%}{124.78 (A)}{2404}{12436.19}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{2559}{70\%}{16.10 (E)}{8634}{397.78}{}
\row{\IfcBugStoreNoValueTaint}{2876}{69\%}{0.33 (E)}{60481}{2.43}{}
\row{\IfcBugJumpNoRaisePc}{2552}{66\%}{5.26 (E)}{15111}{161.50}{}
\row{\IfcBugJumpLowerPc}{2263}{69\%}{104.62 (A)}{2867}{11825.28}{}
\row{\IfcBugStoreNoPcTaint}{2157}{70\%}{873.79 (A)}{341}{642248.07}{}
\row{\IfcBugAllowWriteDownWithHighPc}{2151}{70\%}{717.72 (A)}{417}{449563.72}{}
\row{\IfcBugCallNoRaisePc}{2251}{69\%}{115.15 (A)}{2605}{15014.01}{}
\row{\IfcBugReturnNoTaint}{2138}{70\%}{1490.80 (A)}{201}{1833154.92}{}
\row{\IfcBugValueOrVoidOnReturn}{2127}{70\%}{1811.66 (A)}{165}{3775976.00}{}
\row{\IfcBugPopPopsReturns}{2068}{70\%}{16107.22 (A)}{18}{340349412.50}{}
\means{}{1526.75}{46.48}{0.31}
\extrabuginfo{InstrsCally}{\PropEENI}{EquivLow}{StartQuasiInitial}{\GenByExec2}{True}{300sec}{4000}{Thu Mar 28 19:08:37 EDT 2013}
\averagespeed{2391}
\averagediscrate{69\%}


==> exp-Cally-EENI-Mem-Initial-ByExec2-True.tex <==
\gdef\bugtableinfo{../picopaper/exp-Cally-EENI-Mem-Initial-ByExec2-True.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{2766}{66\%}{37.07 (E)}{5690}{1845.57}{}
\row{\IfcBugPushNoTaint}{2867}{59\%}{0.22 (E)}{73907}{1.42}{}
\row{\IfcBugLoadNoTaint}{2758}{65\%}{155.07 (A)}{1934}{20608.26}{}
\row{\IfcBugStoreNoPointerTaint}{2737}{65\%}{20018.67 (A)}{14}{1144180762.90}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{2911}{67\%}{13.02 (E)}{9602}{311.55}{}
\row{\IfcBugStoreNoValueTaint}{3019}{68\%}{0.35 (E)}{58545}{2.72}{}
\row{\IfcBugJumpNoRaisePc}{2812}{61\%}{48.84 (E)}{4957}{2873.66}{}
\row{\IfcBugJumpLowerPc}{2784}{64\%}{2421.99 (A)}{122}{5740052.41}{}
\row{\IfcBugStoreNoPcTaint}{2765}{65\%}{13289.39 (A)}{22}{91172200.23}{}
\row{\IfcBugAllowWriteDownWithHighPc}{2743}{65\%}{1047.56 (A)}{286}{835168.92}{}
\row{\IfcBugCallNoRaisePc}{2763}{64\%}{3919.08 (A)}{73}{12957670.60}{}
\row{\IfcBugReturnNoTaint}{2749}{65\%}{12804.51 (A)}{22}{354360539.50}{}
\row{\IfcBugValueOrVoidOnReturn}{2741}{65\%}{69081.50 (A)}{1}{---}{}
\row{\IfcBugPopPopsReturns}{2714}{65\%}{---}{0}{---}{}
\means{}{---}{---}{1.72}
\extrabuginfo{InstrsCally}{\PropEENI}{EquivMem}{StartInitial}{\GenByExec2}{True}{300sec}{4000}{Thu Mar 28 19:03:52 EDT 2013}
\averagespeed{2795}
\averagediscrate{65\%}


==> exp-Cally-LLNI-Low-QuasiInitial-ByExec2-True.tex <==
\gdef\bugtableinfo{../picopaper/exp-Cally-LLNI-Low-QuasiInitial-ByExec2-True.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{1451}{0\%}{0.36 (E)}{57373}{3.22}{}
\row{\IfcBugPushNoTaint}{1165}{0\%}{0.01 (E)}{293802}{0.02}{}
\row{\IfcBugLoadNoTaint}{1452}{0\%}{1.14 (E)}{32380}{14.11}{}
\row{\IfcBugStoreNoPointerTaint}{1105}{0\%}{84.08 (A)}{3564}{6149.55}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{1343}{0\%}{5.25 (E)}{15116}{111.37}{}
\row{\IfcBugStoreNoValueTaint}{1442}{0\%}{0.08 (E)}{125267}{0.28}{}
\row{\IfcBugJumpNoRaisePc}{1350}{0\%}{0.08 (E)}{125555}{0.29}{}
\row{\IfcBugJumpLowerPc}{1337}{0\%}{2.80 (E)}{20688}{73.88}{}
\row{\IfcBugStoreNoPcTaint}{1058}{0\%}{232.19 (A)}{1292}{51687.42}{}
\row{\IfcBugAllowWriteDownWithHighPc}{1056}{0\%}{177.75 (A)}{1686}{29708.06}{}
\row{\IfcBugCallNoRaisePc}{1276}{0\%}{5.97 (E)}{14181}{204.77}{}
\row{\IfcBugReturnNoTaint}{1040}{0\%}{337.74 (A)}{888}{111185.32}{}
\row{\IfcBugValueOrVoidOnReturn}{1033}{0\%}{396.37 (A)}{756}{150103.77}{}
\row{\IfcBugPopPopsReturns}{1023}{0\%}{1828.56 (A)}{164}{3644935.30}{}
\means{}{219.46}{7.69}{0.14}
\extrabuginfo{InstrsCally}{\PropLLNI}{EquivLow}{StartQuasiInitial}{\GenByExec2}{True}{300sec}{4000}{Thu Mar 28 18:57:30 EDT 2013}
\averagespeed{1224}
\averagediscrate{0\%}


==> exp-Cally-SSNI-Full-Arbitrary-Naive-True.tex <==
\gdef\bugtableinfo{../picopaper/exp-Cally-SSNI-Full-Arbitrary-Naive-True.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{9880}{46\%}{0.24 (E)}{70541}{2.23}{}
\row{\IfcBugPushNoTaint}{7646}{42\%}{1.06 (E)}{33586}{22.76}{}
\row{\IfcBugLoadNoTaint}{7106}{41\%}{3.25 (E)}{19230}{81.95}{}
\row{\IfcBugStoreNoPointerTaint}{5870}{38\%}{289.63 (A)}{1034}{80355.31}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{6137}{39\%}{31.11 (E)}{6211}{1728.86}{}
\row{\IfcBugStoreNoValueTaint}{8567}{43\%}{0.73 (E)}{40503}{10.14}{}
\row{\IfcBugJumpNoRaisePc}{8807}{41\%}{1.45 (E)}{28739}{34.54}{}
\row{\IfcBugJumpLowerPc}{9524}{41\%}{16.88 (E)}{8431}{868.97}{}
\row{\IfcBugStoreNoPcTaint}{9511}{39\%}{8.77 (E)}{11697}{334.22}{}
\row{\IfcBugAllowWriteDownWithHighPc}{10211}{39\%}{2.26 (E)}{23061}{52.66}{}
\row{\IfcBugCallNoRaisePc}{9267}{41\%}{31.71 (E)}{6152}{1826.00}{}
\row{\IfcBugReturnNoTaint}{8708}{38\%}{1110.09 (A)}{270}{1095285.69}{}
\row{\IfcBugValueOrVoidOnReturn}{8725}{38\%}{1194.30 (A)}{251}{1342223.15}{}
\row{\IfcBugPopPopsReturns}{8894}{37\%}{30.68 (E)}{6254}{1795.16}{}
\means{}{194.44}{12.87}{1.71}
\extrabuginfo{InstrsCally}{\PropSSNI}{EquivFull}{StartArbitrary}{\GenNaive}{True}{300sec}{4000}{Thu Mar 28 19:30:26 EDT 2013}
\averagespeed{8490}
\averagediscrate{40\%}


==> exp-Cally-SSNI-Full-Arbitrary-TinySSNI-True.tex <==
\gdef\bugtableinfo{../picopaper/exp-Cally-SSNI-Full-Arbitrary-TinySSNI-True.tex}%
% Format = bug & #tests/sec & discard ratio & mean time to failure
\row{\IfcBugArithNoTaint}{13368}{9\%}{0.11 (E)}{106051}{0.57}{}
\row{\IfcBugPushNoTaint}{13188}{8\%}{0.06 (E)}{143683}{0.23}{}
\row{\IfcBugLoadNoTaint}{13327}{9\%}{0.61 (E)}{44519}{7.22}{}
\row{\IfcBugStoreNoPointerTaint}{16717}{9\%}{16.32 (E)}{8576}{781.24}{}
\row{\IfcBugAllowWriteDownThroughHighPtr}{19983}{8\%}{0.33 (E)}{59931}{3.09}{}
\row{\IfcBugStoreNoValueTaint}{19890}{8\%}{0.03 (E)}{212987}{0.07}{}
\row{\IfcBugJumpNoRaisePc}{19937}{9\%}{0.09 (E)}{117561}{0.42}{}
\row{\IfcBugJumpLowerPc}{20137}{11\%}{0.49 (E)}{49396}{5.54}{}
\row{\IfcBugStoreNoPcTaint}{20212}{9\%}{1.13 (E)}{32596}{18.85}{}
\row{\IfcBugAllowWriteDownWithHighPc}{20070}{8\%}{0.29 (E)}{64798}{2.56}{}
\row{\IfcBugCallNoRaisePc}{20134}{11\%}{0.62 (E)}{44076}{7.57}{}
\row{\IfcBugReturnNoTaint}{20233}{9\%}{3.10 (E)}{19662}{82.91}{}
\row{\IfcBugValueOrVoidOnReturn}{20465}{10\%}{4.56 (E)}{16215}{138.48}{}
\row{\IfcBugPopPopsReturns}{20040}{9\%}{0.42 (E)}{53318}{4.36}{}
\means{}{2.01}{0.47}{0.15}
\extrabuginfo{InstrsCally}{\PropSSNI}{EquivFull}{StartArbitrary}{\GenTinySSNI}{True}{300sec}{4000}{Thu Mar 28 19:10:09 EDT 2013}
\averagespeed{18407}
\averagediscrate{9\%}


==> expsettings.tex <==
% Automatically generated -- do not modify by hand


==> genbasic.tex <==
% This is hand-built for now; should be automatically generated at some point

            & Naive && & Longer && & Weighted && & Gen-By-Exec \\
\midrule
\rn{Add*}   & 567   & 0.3s & 100\% & 299   & 0.3s & 100\% & 319   & 0.4s  & 100\% & 16   & 0.4s & 100\%  \\
\rn{Push*}  & 3666  & 0.8s & 100\% & 4613  & 1.0s & 100\% & 162   & 0.2s &  100\% & 7    & 0.2s & 100\%  \\
\rn{Load*}  & 28560 & 5.0s & 5\%   & 27652 & 6.0s & 20\%  & 30000 & 7.8s &    0\% & 2474 & 8.1s &  100\% \\
\rn{Store*} & 24468 & 4.4s & 30\%  & 18658 & 4.0s & 60\%  & 25219 & 7.4s &   35\% & 8718 & 24.2s & 100\% 


==> prof-Extended-LLNI-SSNI.tex <==
\begingroup
\newcommand*{\none}{\text{---}}
\newcommand*{\h}[1]{\multicolumn{1}{r}{\Pbox{#1}}}
\newcommand*{\RI}[1]{\textbf{\textit{#1}}}
\newcommand*{\I}[1]{\ifmmode\mathbf{#1}\else\textbf{#1}\fi}
\newcommand*{\Inone}{\text{\textbf{---}}}
\begin{tabular}{@{}l*8{mr}@{}}
\toprule
MTTF                 & \h{SSNI\\(naive)} & \h{SSNI}   & \h{EENI}    & \h{LLNI\\(unopt)} & \h{LLNI\\(naive)} & \h{LLNI}   & \h{MSNI\\(naive)} & \h{MSNI}  \\
\midrule
\ii{Mlab}            & 17.90             & 25.76      & 621.67      & 14.48             & 11.55             & 16.14      & 13.30             & 19.14     \\
\ii{Bcall}           & 8.91              & 12.34      & 434.55      & 20.32             & 15.95             & 22.78      & 9.05              & 11.46     \\
\ii{Bcall}           & 6.58              & 9.20       & 76.67       & 55.08             & 39.66             & 81.78      & 2.42              & 3.82      \\
\ii{Bcall}           & 12.09             & 19.12      & 1622.50     & 7.17              & 5.71              & 7.43       & 6.67              & 8.73      \\
\ii{Bret}            & 30.02             & 19.44      & 301.35      & 1030.00           & 19.01             & 12.32      & 22.15             & 14.38     \\
\ii{Bret}            & 128.06            & 81.00      & 817.50      & 658.33            & 130.61            & 80.65      & 169.44            & 104.13    \\
\ii{Bret}            & 13.04             & 9.00       & 134.68      & 12.00             & 9.26              & 6.26       & 10.93             & 7.60      \\
\ii{Bret}            & 9.62              & 5.90       & 376.39      & 13.66             & 10.21             & 6.96       & 13.67             & 7.90      \\
\ii{Noop}            & 5.24              & 6.91       & 78.86       & 1.07              & 4.52              & 6.28       & 5.08              & 7.48      \\
\ii{Binop}           & 60.81             & 79.70      & 598.67      & 26.24             & 20.63             & 25.27      & 26.31             & 33.50     \\
\ii{Binop}           & 64.02             & 94.89      & 434.78      & 26.71             & 19.34             & 26.77      & 24.80             & 31.59     \\
\ii{Jump}            & 40.63             & 54.57      & 64.00       & 18.95             & 16.76             & 26.45      & 16.53             & 31.90     \\
\ii{Jump}            & 13.11             & 19.93      & 1851.33     & 7.81              & 5.43              & 7.24       & 6.87              & 8.61      \\
\ii{Bnz}             & 17.53             & 25.05      & \none       & 39.42             & 36.07             & 48.45      & 41.96             & 58.28     \\
\ii{Bnz}             & 49.17             & 63.55      & 75.68       & 17.41             & 13.75             & 22.84      & 16.52             & 28.32     \\
\ii{Load}            & 68.86             & 77.77      & 617.71      & 43.99             & 29.58             & 32.54      & 39.68             & 49.39     \\
\ii{Load}            & 55.75             & 48.97      & 1863.33     & 100.17            & 72.34             & 78.69      & 19.91             & 21.52     \\
\ii{Load}            & 77.94             & 76.90      & 1332.86     & 76.23             & 53.14             & 49.85      & 64.72             & 69.40     \\
\ii{Store}           & 66.42             & 29.61      & 1307.78     & 130.26            & 22.14             & 9.30       & 24.67             & 11.30     \\
\ii{Store}           & 29.48             & 14.77      & \none       & \none             & \none             & 583.33     & 12.84             & 7.33      \\
\ii{Store}           & 111.84            & 57.28      & 1185.83     & 76.79             & 54.86             & 24.81      & 68.53             & 27.39     \\
\ii{Write}           & 101.44            & 55.73      & \none       & \none             & \none             & 580.00     & 39.63             & 25.23     \\
\ii{Write}           & 222.29            & 129.64     & 3366.67     & 272.87            & 63.59             & 38.27      & 105.09            & 38.18     \\
\ii{Write}           & 180.59            & 87.60      & \none       & \none             & 102.61            & 40.95      & 108.58            & 49.33     \\
\ii{Write}           & 17.29             & 8.47       & 335.75      & 43.98             & 30.23             & 16.69      & 8.58              & 4.52      \\
\ii{Update}          & 189.03            & 198.95     & \none       & \none             & 141.72            & 95.83      & 256.58            & 100.65    \\
\ii{Update}          & 126.99            & 69.62      & \none       & \none             & \none             & \none      & 53.28             & 36.50     \\
\ii{Update}          & 150.77            & 80.54      & \none       & \none             & 109.63            & 47.48      & 130.96            & 65.67     \\
\ii{Update}          & 253.04            & 180.07     & 1864.17     & 614.67            & 102.64            & 61.58      & 149.29            & 67.36     \\
\ii{Update}          & 367.78            & 169.15     & 2993.33     & 332.56            & 259.14            & 132.18     & 262.11            & 127.27    \\
\ii{Alloc}           & 27.07             & 29.32      & 13.10       & 23.51             & 16.35             & 18.09      & 20.46             & 20.53     \\
\ii{Alloc}           & 26.59             & 28.83      & 13.92       & 23.61             & 16.55             & 20.39      & 22.20             & 21.00     \\
\ii{Psetoff}         & 31.17             & 42.97      & 220.22      & 25.12             & 18.80             & 25.08      & 22.82             & 29.74     \\
\ii{Psetoff}         & 32.03             & 52.02      & 579.11      & 18.91             & 14.28             & 18.86      & 17.31             & 20.21     \\
\ii{Pgetoff}         & 17.18             & 24.45      & 227.05      & 10.67             & 8.36              & 11.20      & 10.12             & 12.79     \\
\ii{Msize}           & 31.76             & 47.78      & 406.38      & 30.52             & 23.50             & 35.64      & 28.70             & 40.12     \\
\ii{Msize}           & 49.81             & 69.31      & 1053.33     & 42.73             & 31.26             & 42.88      & 34.05             & 49.88     \\
\ii{Mov}             & 10.19             & 14.33      & 149.85      & 8.52              & 6.95              & 8.88       & 8.68              & 10.60     \\
\midrule
\RI{Arithmetic mean} & \I{71.63}         & \I{55.80}  & \Inone      & \Inone            & \Inone            & \Inone     & \I{49.85}         & \I{33.76} \\
\RI{Geometric mean}  & \I{24.07}         & \I{24.70}  & \I{121.18}  & \I{14.24}         & \I{16.81}         & \I{18.91}  & \I{15.64}         & \I{16.03} \\
\bottomrule
\end{tabular}
\endgroup


==> prof-Initial-ByExec-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
11.17%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 11.17}\\\midrule
99\% & halt \\
\end{tabular}
\fi%


==> prof-Initial-ByExec-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
11.62%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 11.62}\\\midrule
99\% & halt \\
\end{tabular}
\fi%


==> prof-Initial-Naive-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
0.51%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 0.51}\\\midrule
76\% & stack underflow \\
21\% & halt \\
1\% & load or store out of range \\
\end{tabular}
\fi%


==> prof-Initial-Weighted-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
3.39%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 3.39}\\\midrule
46\% & halt \\
37\% & stack underflow \\
11\% & load or store out of range \\
4\% & sensitive upgrade \\
\end{tabular}
\fi%


==> prof-QuasiInitial-ByExec-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
11.74%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 11.74}\\\midrule
99\% & halt \\
\end{tabular}
\fi%


==> prof-QuasiInitial-ByExec-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
12.49%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 12.49}\\\midrule
99\% & halt \\
\end{tabular}
\fi%


==> prof-QuasiInitial-Naive-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
1.27%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 1.27}\\\midrule
60\% & load or store out of range \\
32\% & halt \\
7\% & stack underflow \\
\end{tabular}
\fi%


==> prof-QuasiInitial-Naive-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
2.65%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 2.65}\\\midrule
52\% & halt \\
28\% & load or store out of range \\
10\% & sensitive upgrade \\
8\% & stack underflow \\
\end{tabular}
\fi%


==> prof-QuasiInitial-Sequence-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
3.71%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 3.71}\\\midrule
51\% & halt \\
39\% & load or store out of range \\
7\% & sensitive upgrade \\
2\% & stack underflow \\
\end{tabular}
\fi%


==> prof-QuasiInitial-Sequence-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
4.51%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 4.51}\\\midrule
60\% & halt \\
25\% & load or store out of range \\
11\% & sensitive upgrade \\
2\% & stack underflow \\
\end{tabular}
\fi%


==> prof-QuasiInitial-Weighted-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
2.12%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 2.12}\\\midrule
49\% & load or store out of range \\
46\% & halt \\
3\% & stack underflow \\
\end{tabular}
\fi%


==> prof-QuasiInitial-Weighted-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling
\ifonlylen%
3.41%
\else%
\begin{tabular}{rl}
\multicolumn{2}{l}{Average number of execution steps: 3.41}\\\midrule
66\% & halt \\
22\% & load or store out of range \\
7\% & sensitive upgrade \\
4\% & stack underflow \\
\end{tabular}
\fi%


==> profvar-Initial-ByExec-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
11.17%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 11.17 & 9.55\\\midrule
80\% & halt & halt \\
18\% & halt & load or store out of range \\
\end{tabular}
\fi%


==> profvar-Initial-ByExec-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
11.60%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 11.60 & 11.26\\\midrule
95\% & halt & halt \\
3\% & halt & load or store out of range \\
1\% & halt & sensitive upgrade \\
\end{tabular}
\fi%


==> profvar-Initial-Naive-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
0.46%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 0.46 & 0.48\\\midrule
74\% & stack underflow & stack underflow \\
21\% & halt & halt \\
3\% & load or store out of range & load or store out of range \\
\end{tabular}
\fi%


==> profvar-Initial-Naive-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
0.53%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 0.53 & 0.53\\\midrule
76\% & stack underflow & stack underflow \\
21\% & halt & halt \\
1\% & load or store out of range & load or store out of range \\
\end{tabular}
\fi%


==> profvar-Initial-Sequence-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
3.87%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 3.87 & 3.69\\\midrule
35\% & halt & halt \\
24\% & load or store out of range & load or store out of range \\
20\% & stack underflow & stack underflow \\
7\% & sensitive upgrade & load or store out of range \\
5\% & sensitive upgrade & sensitive upgrade \\
2\% & load or store out of range & sensitive upgrade \\
2\% & halt & load or store out of range \\
1\% & load or store out of range & halt \\
\end{tabular}
\fi%


==> profvar-Initial-Sequence-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
4.23%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 4.23 & 4.25\\\midrule
40\% & halt & halt \\
21\% & stack underflow & stack underflow \\
18\% & load or store out of range & load or store out of range \\
14\% & sensitive upgrade & sensitive upgrade \\
2\% & load or store out of range & sensitive upgrade \\
1\% & sensitive upgrade & load or store out of range \\
\end{tabular}
\fi%


==> profvar-Initial-Weighted-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
2.71%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 2.71 & 2.84\\\midrule
39\% & halt & halt \\
35\% & stack underflow & stack underflow \\
20\% & load or store out of range & load or store out of range \\
2\% & load or store out of range & sensitive upgrade \\
1\% & load or store out of range & halt \\
\end{tabular}
\fi%


==> profvar-Initial-Weighted-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
3.37%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 3.37 & 3.41\\\midrule
45\% & halt & halt \\
37\% & stack underflow & stack underflow \\
9\% & load or store out of range & load or store out of range \\
4\% & sensitive upgrade & sensitive upgrade \\
1\% & load or store out of range & sensitive upgrade \\
\end{tabular}
\fi%


==> profvar-QuasiInitial-ByExec-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
11.73%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 11.73 & 9.97\\\midrule
78\% & halt & halt \\
19\% & halt & load or store out of range \\
\end{tabular}
\fi%


==> profvar-QuasiInitial-ByExec-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
12.50%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 12.50 & 11.39\\\midrule
86\% & halt & halt \\
7\% & halt & sensitive upgrade \\
5\% & halt & load or store out of range \\
\end{tabular}
\fi%


==> profvar-QuasiInitial-Naive-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
1.29%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 1.29 & 1.51\\\midrule
52\% & load or store out of range & load or store out of range \\
32\% & halt & halt \\
7\% & stack underflow & stack underflow \\
3\% & load or store out of range & sensitive upgrade \\
3\% & load or store out of range & halt \\
\end{tabular}
\fi%


==> profvar-QuasiInitial-Naive-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
2.70%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 2.70 & 2.75\\\midrule
48\% & halt & halt \\
22\% & load or store out of range & load or store out of range \\
8\% & stack underflow & stack underflow \\
5\% & sensitive upgrade & sensitive upgrade \\
2\% & sensitive upgrade & load or store out of range \\
2\% & sensitive upgrade & halt \\
2\% & load or store out of range & sensitive upgrade \\
2\% & load or store out of range & halt \\
2\% & halt & sensitive upgrade \\
1\% & halt & load or store out of range \\
\end{tabular}
\fi%


==> profvar-QuasiInitial-Sequence-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
3.77%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 3.77 & 3.53\\\midrule
44\% & halt & halt \\
34\% & load or store out of range & load or store out of range \\
5\% & halt & load or store out of range \\
4\% & sensitive upgrade & load or store out of range \\
2\% & stack underflow & stack underflow \\
2\% & load or store out of range & sensitive upgrade \\
2\% & load or store out of range & halt \\
1\% & sensitive upgrade & sensitive upgrade \\
\end{tabular}
\fi%


==> profvar-QuasiInitial-Sequence-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
4.56%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 4.56 & 4.62\\\midrule
56\% & halt & halt \\
21\% & load or store out of range & load or store out of range \\
6\% & sensitive upgrade & sensitive upgrade \\
2\% & stack underflow & stack underflow \\
2\% & sensitive upgrade & halt \\
2\% & load or store out of range & sensitive upgrade \\
2\% & halt & sensitive upgrade \\
1\% & sensitive upgrade & load or store out of range \\
1\% & load or store out of range & halt \\
1\% & halt & load or store out of range \\
\end{tabular}
\fi%


==> profvar-QuasiInitial-Weighted-False.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
2.15%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 2.15 & 2.39\\\midrule
45\% & halt & halt \\
42\% & load or store out of range & load or store out of range \\
4\% & stack underflow & stack underflow \\
3\% & load or store out of range & sensitive upgrade \\
3\% & load or store out of range & halt \\
\end{tabular}
\fi%


==> profvar-QuasiInitial-Weighted-True.tex <==
% Format = bug & #tests/sec & discard ratio & #finds/sec
% Profiling variations
\ifonlylen%
3.49%
\else%
\begin{tabular}{rll}
 & Generated & Variation \\\midrule
 Steps & 3.49 & 3.56\\\midrule
63\% & halt & halt \\
18\% & load or store out of range & load or store out of range \\
4\% & stack underflow & stack underflow \\
3\% & sensitive upgrade & sensitive upgrade \\
2\% & load or store out of range & sensitive upgrade \\
2\% & load or store out of range & halt \\
1\% & sensitive upgrade & load or store out of range \\
1\% & sensitive upgrade & halt \\
1\% & halt & sensitive upgrade \\
1\% & halt & load or store out of range \\
\end{tabular}
\fi%


==> texdirectives.tex <==
\draftfalse\fulltrue\techreptrue

